Carbon Emissions of Quantum Circuit Simulation: More than You Would Think

The rapid advancement of quantum hardware brings a host of research opportunities and the potential for quantum advantages across numerous fields. In this landscape, quantum circuit simulations serve as an indispensable tool by emulating quantum behavior on classical computers. They offer easy access, noise-free environments, and real-time observation of quantum states. However, the sustainability aspect of quantum circuit simulation is yet to be explored. In this paper, we introduce for the first time the concept of environmental impact from quantum circuit simulation. We present a preliminary model to compute the CO2e emissions derived from quantum circuit simulations. Our results indicate that large quantum circuit simulations (43 qubits) could lead to CO2e emissions 48 times greater than training a transformer machine learning model.

==> challenge.tex <==
\section{challenge and motivation}
\input{FigureText/motivation}

This section will demonstrate our observations of current quantum machine learning and the existing challenges that limit further study in this field that motivates us in this research.
\subsection{The Importance of Non-linearity During the Computation Circuit}
The strength of deep learning is its ability to solve complex problems by learning the complicated transformation between inputs and outputs through different neural network layers with non-linear functions. On the other hand, despite recent advances in quantum machine learning, one of the major challenges is the ability to effectively handle nonlinearity. The model used in quantum machine learning itself is basically a linear transformation now given that the computation circuit doesn't involve any non-linearity but only matrix multiplication. However, many real-world phenomena cannot be adequately modeled using linear models.

Motivated by that, the research on non-linearity in Quantum Machine Learning becomes more important in order to enhance the ability of models. Therefore it can finally extend the frontier of this area in solving more difficult problems. 

\subsection{Unfair Comparison between Classical ML and Quantum ML}
The current comparison between Classical and Quantum in machine learning is not fair. For example, if we are using the MNIST dataset to do a classification task, we can design both the Classical model such as MLP and the Quantum model such as VQC with the same number of parameters. Although we can evaluate and observe their performance directly, it is not a fair comparison since the same number of parameters doesn't imply that the model can gain the same enhancement in their ability to learn the patterns between input and output as there should be more factors that can lead the models' expressibility. We can see from Figure \ref{fig: motivation} that the performances of classical models become better as increase the number of parameters, while VQC meets the bottleneck and can barely gain benefit from the increase. It is not fair to compare quantum machine learning models with classical machine learning models without considering the bottleneck of VQC.


This can also be observed by contrasting the linear model and MLP; the latter's ability to handle complex datasets is attributed to its more complex network structure with additional hidden layers and activation functions. Therefore, a rigorous analysis of the VQC model's nature is required to ensure a fair comparison with classical models, and a comparison of their nonlinear characteristics can be an insightful perspective to consider.


\subsection{Quantum Model Design Needs Benchmarking}
There is a lack of an evaluator in the design of the quantum machine learning model to evaluate the given design's approximation.
As mentioned before, there can be several factors that have an influence on the ability to approximate the nonlinear relationship between inputs and outputs for a given VQC design such as the structure of the VQC design and the number of parameters used in VQC. However, it is still unclear how a model can benefit from the different adjustments and designs, while there is a high cost in testing whether a VQC model can achieve the desired performance on real-world complex datasets with noise.

Motivated by this, there is a need for benchmarking quantum machine learning models on their ability to handle nonlinearity, which can contribute in several ways:
\begin{itemize}
    \item Identify the strengths and weaknesses of different quantum machine learning models in dealing with nonlinearity. This information can guide the development of new models or the improvement of existing ones.
    \item Provide a quantitative measure of the performance of quantum machine learning models on nonlinear tasks, which can help researchers evaluate and compare different models.    
    \item The benchmarking results can also provide insights into the types of problems that quantum machine learning models are well-suited for and those that may require further development. This can help guide the selection of appropriate quantum machine learning models for real-world applications.
    
\end{itemize}


% \subsection{Lack of Datasets in Analyzing the Nonlinearity in Quantum Models}
% Although the study of nonlinearity in quantum machine learning is beneficial to this area, there still remain some challenges. First, there is a lack of datasets with nonlinearity in quantum ML because simple datasets such as MNIST can be linearly separable while complex datasets require too many qubits, which is now not possible. 

% Motivated by this, generating a series of datasets with nonlinearity can help users easily evaluate their model within acceptable time and limited resources.



% \subsection{High Cost on Evaluating Models on Certain Datasets}
% \input{FigureText/motivation_C}
% There is a high cost on testing whether a VQC model can achieve the desired performance on complex datasets with noise. Although we can increase the parameters of VQC as it enhances the model's ability to capture the complex relationship between input and output, it also increases the risk of overfitting on datasets, especially with noise. As shown in Figure \ref{fig: motivation_C}, the dataset with noise is a polynomial of two variables with each term's degree being 8. The performance becomes poor as we maximize the parameters to make the model too complex. Also, it still remains unclear on how to efficiently analyze a quantum model's ability to handle nonlinearity.

% Motivated by this, it is necessary to have a system tool that can give a thorough analysis of a given quantum learning model design. It can help the users to better evaluate their models and have a better understanding on the level of non-linearity achieved by them. Therefore, users can make wise decisions on the choices of models or update accordingly based on what kinds of problems they can solve.

% \subsection{Lack of Effective Method to Adding Nonlinearity}
% As mentioned above, the computation circuit of quantum machine learning model itself is linear transformation, which limits its ability to handel more complex datasets. It also influences the validation of the proposed evaluator.

% Motivated by this, we propose a novel data encoder that can bring the nonlinearity into the VQC model.
\clearpage
